Simulated Human Learning in a Dynamic, Partially-Observed, Time-Series Environment

While intelligent tutoring systems (ITSs) can use information from past students to personalize instruction, each new student is unique. Moreover, the education problem is inherently difficult because the learning process is only partially observable. We therefore develop a dynamic, time-series environment to simulate a classroom setting, with student-teacher interventions - including tutoring sessions, lectures, and exams. In particular, we design the simulated environment to allow for varying levels of probing interventions that can gather more information. Then, we develop reinforcement learning ITSs that combine learning the individual state of students while pulling from population information through the use of probing interventions. These interventions can reduce the difficulty of student estimation, but also introduce a cost-benefit decision to find a balance between probing enough to get accurate estimates and probing so often that it becomes disruptive to the student. We compare the efficacy of standard RL algorithms with several greedy rules-based heuristic approaches to find that they provide different solutions, but with similar results. We also highlight the difficulty of the problem with increasing levels of hidden information, and the boost that we get if we allow for probing interventions. We show the flexibility of both heuristic and RL policies with regards to changing student population distributions, finding that both are flexible, but RL policies struggle to help harder classes. Finally, we test different course structures with non-probing policies and we find that our policies are able to boost the performance of quiz and midterm structures more than we can in a finals-only structure, highlighting the benefit of having additional information.

==> future.tex <==
% \section{Future Work}

% \subsection{Collaborative Education}
% From these collaborative games, we want to extend into the collaborative education space, similar to the setup described in the motivating example in Section \ref{sec:edu} in the context that education is effectively a collaborative game. 

% Ultimately, much of the setup is the same. We want to incrementally move from this simple collaborative game in Sets into something that increasingly resembles an actual educational space. We still have an estimation task described in Equation \ref{eq:problem} and understand how various types of interventions can change the human state dynamics $\prob{h_{t+1} \vert h_{1:t}, o^e_{1:t}, r^e_{1:t}}$ (intervention assumed to be included in the observation) so that we have the most reward. From this, we can first do student emulation via causal generative models we have researched \cite{causalvae}. 

% Then, we can also begin to understand more complex educational systems. For instance, while the tutoring system has nice properties, we can also extend this further to aid a teacher of multiple students. In this manner, these problems can have the teaching agent have actions similar to lecture, which are broadcast to all students for a certain cost and individual interventions at a cost per student. Then, the teaching agent has an incentive to change the possible lecture trajectory if it can reduce the number of individual interventions required. This can also extend to multiple teaching agents (analogous to TAs) that can each have their own states. 

% Similarly, students may be faced with multiple courses, which means that students must appropriately balance the amount of time resources that they have for each course to achieve the same goals. All of these can advise teachers and students how to better allocate their resources. Depending on estimation ability, this can be as detailed as the specific concepts being taught in the class, but can be as broad as just saying there is a problem and more time needs to be present. 

% \subsection{Other Similar Areas of Research}
% There are many approaches to problems that are similar or useful to this problem that we have found but not investigated fully. More notes on topics that may require more reading. 
% \begin{itemize}
% 	\item Control Theory, in particular adaptive dual control problems \cite{controls}. 
% 	\item Information Theory, both in how much information can be estimated through individual actions given underlying distributions.
% 	\item Federated learning shares many parallels to this problem. We have so far framed it as a transfer learning problem from the perspective of federated learning, but have not fully explored the techniques \cite{federated}. In this case, we do not necessarily have as much concern about privacy. In fact within a course there is no need for privacy at all. This may be different when applied to multiple different courses in multiple institutions. 
% 	\item Meta-learning. We care a lot about how quickly we can determine more optimal actions from very few data points. This is similar to some of the meta-learning literature \cite{maml}. 
% \end{itemize}

==> prob-statement.tex <==
% TODO following was just pasted for now. 

\chapter{Problem Statement}

\section{Motivation}
Recent years have enlightened many more of the general public of the current state and the future potential of artificial intelligence (AI) in our society. 
In light of this new frontier of AI, we've come to realize that an important area of research is to understand how to interface the use of AI with humans.
Examples can be seen in all sorts of examples, such as self-driving cars, medical diagnosis, and even in education. 
AI has the potential to be extremely helpful to humans, but the blackbox nature of AI can also be hard to accept for many people and dangerous in extreme cases.
Thus, we would like to investigate ways to incorporate explainability and human interaction into the use of AI. 

% this is something generated completely differently. 
In particular, the field of reinforcement learning (RL) has been a major driving force in the development of AI. 
RL has been used to solve many problems, such as playing games \cite{alphago, alphastar, alphazero}, robotics \cite{robotics}, and even medical applications \cite{medical}. However, there are still many problems that RL cannot solve. 
In particular, RL is not sample efficient, and requires a large amount of data to learn. Furthermore, RL is not robust to changes in the environment, and can easily fail when the environment changes. Finally, RL is not interpretable, and it is difficult to understand why the agent makes certain decisions.


The problem is formulated based on the reinforcement learning (RL) terminology. For simplicity, we 
At first glance, the problem is effectively a partially-observed Markov decision process (POMDP). 
However, in most cases, we cannot expect the Markovian assumption to hold true. Plus, with partial observability, 
any deviation from the ground truth can quickly degrade prediction performance \cite{RLBook}. In general, with 
too little information, the agent cannot learn the dynamics of the environment.

Thus, we would like to specify a realistic set of rules for our environment, which has a fairly strict set of rules or constraints. 
Within the confines of the rules, we have different actors. These actors need not be symmetric, i.e. they need not have the same state space, action space or objective, but they must operate in the same constraints of the problem space. 
Typically we focus our efforts on one actor, which we call the agent, and the other actor(s) is part of the environment. 
Instead of making this problem a multi-agent problem, we instead deem the human actor as part of the environment. 
In our case, we interchangeably call the agent the ``bot" and the environment actor the ``human." 
Then, we normally 
And, based on this, the objective of the agent is both to achieve an objective in the problem space that is usually common or similar to the human's and to achieve an understanding of the environment's actor. 
Therefore, there are actually two components to consider in the environment space: the problem state and the actor state. 
In particular, the actor state can influence how the problem state dynamics evolve. 
% This is because we want to focus on the agent's ability to understand the environment, and not the environment's ability to understand the agent.
Because the environment is based on some human, we assume the environment to be non-stationary, but follows some causal set of human-understandable set of principles. 

In general, this non-Markovian ``mind-reading" problem is intractable. 
However, we make one further assumption that the agent is able to perform interventions specifically to get information about the environment.
Finally, we also assume that actions are non-catostrophic, i.e. the agent can always recover from any action that it takes and that the agent does not always need to take a theoretically optimal action. % hm?
Thus, at different points in time, we can reduce the uncertainty of the unobserved environment state to better choose future actions. 
With the combination of gaining information and the constraints on the environment, we can view the problem as a causal inference problem, where the agent is trying to infer the environment's state based on the interventions that it performs.
This ends up primarily becoming a problem of how much information is gained through interaction and what qualtiy of estimation this information can provide. 
In terms of data, we may or may not assume that there is an abundance of population data, but we always assume that there is a lack of individual data. 
Instead, based on the population, we form prior knowledge models from which we learn possible dynamics. 
However, we can only choose to create models small enough that estimation is possible within a small number of observations and know how to adjust these models as more data may come in. Our solution to this is to limit the models to discrete sets through the use of causal models. 
By applying causal structures, we want to leverage sample efficiency, and also provide explanations based on causal \textit{interventions} and possible \textit{counterfactual} realities should we have performed other actions, plus a transfer between models based on the level of information gained. 
%This leads to another set of possible problems, as true counterfactuals can never be observed for the individual's state, even if they can be simulated in the problem space. 

Another version of the problem that we would like to investigate comes from the other side. 
Suppose we have two problem spaces that are similar in concepts, but may have different objectives, populations, or rules. 
We hope to see that this causal investigation of the connection between population and individual can also extend to these problem spaces. 
This allows for a very nice understanding of how to transfer learning between problem spaces. 

\section{Education}
\label{sec:edu}
Education, focused particularly in science, technology, engineering, and mathematics (STEM) subjects, acts as our main motivation for this problem. 
In this perspective, the agent takes the role of the \textit{teacher}. 
Here, our environment encapsulates the course, with its proposed structure, the students, and the learning structure. 
Underlying everything, we understand that human learning, especially in STEM subjects comes as a heirarchical causal structure, e.g. calculus builds on algebra, which builds on arithmetic. \jef{Can make a new visual graph for this}
Thus, we can view the learning structure of the environment as a causal graph, where the nodes are concepts and the edges are the dependencies between concepts.
There are other causal structures that we can consider, such as the student's state, which we will discuss later, and the effectiveness of an intervention. 
For instance, whether a student learned a concept at a specific time depends both on whether they are solid in prerequisite material and whether they spent enough time studying the concept.
The amount of time a student can spend can depend on many factors, such as their motivation, which can be affected by interest, health, and social circumstances, their other classes, and their other responsibilities.
In this case, it is in the best interest of students and instructors if there is as much transfer of information as possible to diagnose and alleviate problems earlier on. 
The causal structure of a course is shown in a very rough way in Figure \ref{fig:education-dag}. 

\begin{figure}[htbp]
	\begin{center}
		\input tikz/education.tikz
	\end{center}
	\caption{A time-dynamic DAG of a course from the perspective of the student, where there are time-dependencies going to the right. Each blue node can represent some concept that is being taught in a course (or is a prerequisite). Each red bar represents an intervention, which can be a classwide examination. The student state is dynamic and can have various other effects. }
	\label{fig:education-dag}
\end{figure}

\begin{figure}[htbp]
	\begin{center}
		\input tikz/student.tikz
	\end{center}
	\caption{A simple hypothesized DAG about how a student may produce results for any single concept in a duration of time. Each of the inputs at the top are time dependent. }
	\label{fig:student-dag}
\end{figure}

Students may have the noble goal of achieving knowledge of the course material, but most of the time have the proxy goal of getting a good grade. 
Similarly, professors generally want to educate students in their field, but also have other interests such as research and has limited time as a result. 
Therefore, the agent and the environment have a similar goal, but have asymmetries in both the exact reward function, the information they have access to, and the actions that they can take.

In education, the student can take many actions and their state necessarily changes throughout a course. 
Basic actions are to do the necessities of the class: lecture, homework, and examination. 
However, there are some extra actions, such as those shown in Figure \ref{fig:student-dag}. \jef{There's a good chance that this isn't how I've coded things right now.}
Each of these ``extra" actions has a trade-off for the student for increasing their performance in the class, but has a cost of the time that it takes. 
This can be understood as instantaneous negative rewards for the possibility of obtaining a higher final reward. 
Each student, however, may respond to different inputs differently, making the problem similar to a federated learning task. 
From this example, we can also see the need for an understanding of population and individual responses toward interventions. 
We only get a handful of observations per individual, so we can never get enough information to fully personalize the interventions,
but we can still get a good idea of how to personalize the interventions based on the population. 
However, we also must acknowledge that individuals differ and there can be highly different responses to interventions per sub-population. 

On the other hand, the teacher is usually unaware of the students' states. 
The basic action is to broadcast information to every student in the class, through announcements, lectures, or assignments. 
Lectures and announcements typically don't actually reciprocate much information from the students, but assignments and examinations do.
Each assignment gives a small amount of information and examinations give higher quality information. 
Afterward, there could be individual interventions, such as requesting to come to office hours, which is more effective for the student, but is less efficient from a class performance perspective. 
With increased information, the professor can realize that there is a systematic problem in the class and adjust the class structure to better facilitate the learning, such as doing a remedial lecture or posting review notes. 
As professors have limited time, the increase in information can help them better allocate their time to help the students.
However, without some ability to ``mind read" from observations or provide good interventions, both teachers and students may not understand how well they are doing. 

Finally, obtaining educational data is costly, as it requires manpower to collect and student time. 
Also, the information that we get from students is often limited and not useful due to the fact that students are not sure themselves. 
Most recently, our lab had collected biweekly self-assessment surveys from 79 students in the UCLA ECE 115C class in Spring 2022, only to find out that most students only had the confidence to say they had basic understanding of the concepts being taught. 
This can largely be attributed to a student's constant self-doubt when it comes to concepts without an examination reference point, which is their ultimate goal. 
Therefore, we can only conclude that an increase in examinations could help improve student confidence at the cost of lecture and professor time. 
Thus, based on our problem formulation, this should be investigated in the context of this short-term cost vs. long-term reward. \je{How to best incorporate this information?}

\section{Games}
As we have considered RL as a framework for our problem, we can also consider the problem in the context of games.
Games have been the natural playground for RL, as they are easy to simulate, generally have strong Markovian assumptions, and can be easily adjusted to test different structural hypotheses.
Based on the description of education provided, we can view the teacher-student relationship as a two-player game, where the teacher is the agent and the student is the environment.
Thus, we can use certain toy games as stepping stones to understand the problem better.

In many instances, reinforcement learning (RL) applied to games tends to result in search spaces that heavily rely on minimax strategies or Nash equilibrium solutions. 
When dealing with a scenario akin to minimax, the environment is playing at its optimal level. 
In such a situation where the environment plays optimally, the problem simplifies to a standard non-dynamic RL problem, eliminating the need to estimate the player's state. 
However, this is not the desired outcome for our problem. 
Specifically, the challenge of discovering the human state and winning the game reflects the same balance between exploitation and exploration found in traditional dual control or reinforcement learning problems. Further exploration of the multi-agent RL literature may be beneficial.
\je{Might need to look a bit more into the multi-agent RL literature.}

After testing some competitive games, \textit{collaborative games} fit the problem that we are solving better. 
In adversarial games, the environment is the \textit{opponent}. 
In such an environment, the ideal flow of information between competitors is to have as little as possible.
Thus, the onus on forcing information flow is on the structural design of the game. 
However, it is in both players' best interest to lie and deceive as much as is allowed to by the game, which lowers information quality of actions to the agent.
In the collaborative case, both players are now \textit{partners}. 
The partner does not have an incentive to force dynamics and so the problem results more toward natural dynamics which can be much better behaved. 

Furthermore, games can be easily be adjusted. These adjustments can result in completely new tasks with similar concepts. 
Or, we can use new methods to encode implicit causal information through adding interventions. 
Ultimately, the flexibility of games is a big selling point in their use, as their complexity can start small and increase based on how the rules have been set. 
This justifies the use of different methods of causal understanding of both the game space and the individual space that can transfer much easier between different versions of games. 
Besides just understanding how flexible our causal modeling is, we can also make rule modifications for the explicit purpose of testing interventions. 
\je{Again, may need to do some small amount of work wrt this.}

\section{Medical}
Finally, many of these concepts apply directly to the medical domain. 
Here, the agent would refer to a medical assistant aiding the patient which is the environment. 
In this case, the patient and the assistant have a common goal of successful treatment. 
The agent receives sparse information from the patients, typically only when recording takes place (e.g. when a device is being used). 

In medicine, the environment state is definitely not anywhere close to being fully observed. 
There is the patient's health conditions, of which the improvement is the main goal. 
The agent's actions are the set of recommendations given to the patient. 
In addition, the agent may also want to balance additional costs (specialists' time, possible side effects, actual monetary costs) into the objective. 
However, there is also an additional patient knowledge and treatment state. 
These include more of such concepts as the patient's knowledge of their health conditions, their willingness and motivation to improve their conditions, and other external factors that can influence the patient to change their actions in treatment. 

However, there are some setbacks in the medical domain. First, getting medical data is expensive in money, time, and sometimes urgency. 
We cannot feasibly get interactive experiment data without the help of medical professionals and would have to rely on observational data instead. 
This is further compounded by the requirement of expert information to construct causal models, which may still be noisy and never truly known. 
Finally, models in medicine are still hopelessly complex. 
Even with many of the recent advances, even hypothesizing causal models is a difficult task. 
As we do not have these resources, we do not pursue this application further, except to use insights that come from the field \cite{corpus, NeuralCDE, MedicalIRL, MedicalNeuralCDE}. 


\je{We can add a further subsection purely just about how this applies to human interaction.}

\section{Formal Problem Statement}
The RL environment can be separated into a \textit{Game Space} and \textit{Human Space}.
Consider the game space, defined for two players, denoted $a$ for agent and $e$ for environment. 
For now, we will assume that the game has a predefined fixed structure. 
Each player observes a sequence of observations $\{o^a_t: t \in \{1, \dots, T\}\}, \{o^e_t: t \in \{1, \dots, T\}\}$, 
performs a sequence of actions $\{a^a_t: t \in \{1, \dots, T\}\}, \{a^e_t: t \in \{1, \dots, T\}\}$, 
and receive a sequence of rewards $\{r^a_t : t \in \{1, \dots, T\}\}, \{r^e_t : t \in \{1, \dots, T\}\}$. 
Because the agent and environment do not have to be playing symmetric games, the states and actions do not need to come from the same support. 
Based purely on the game dynamics, $\prob{o^e_{t+1}, r^e_{t+1} \vert o^a_t, a^a_t}$ and $\prob{o^a_{t+1},  r^a_{t+1} \vert o^e_t, a^e_t}$ are some fixed distribution. 
Of course, because the game itself need not stationary, these distributions can be different at different points in time $t$. 

Now, we discuss the unobserved components from the agent's perspective. 
For now we ignore the reward, as that is defined purely based on the game dynamics. 
From the agent's perspective, the game can be reduced using Markovian assumptions on the game to 
\begin{equation}
	\prob{o^a_{t+1} \vert o^a_t, a^a_t} = \sum_{o^e_t, a^e_t} \prob{ o^e_t \vert o^a_t, a^a_t} \prob{a^e_{t} \vert o^e_{t}} \prob{o^a_{t+1} \vert o^e_t, a^e_t}
	\label{eq:markov-breakdown}
\end{equation}
Here, the $t$ indexing assumes that the $t$ time step for the environment comes after the $t$ time step for the agent. 

First, unless the game is fully observed, we only have partial information of $o^e_t$ given $o^a_t$, \textit{i.e.} we can only have some distribution $\prob{o^e_t \vert o^a_t, a^a_t}$. 
The main consideration, though, is that the agent cannot observe the policy $\prob{a^e_{t} \vert o^e_{t}}$, even if we know $o^e_t$. 
Furthermore, we assume in our problems that this policy is dynamic. 
For instance, if we normally assume the self-play minimax solutions, we may assume that $\prob{a^e_{t} \vert o^e_{t}} =\prob{a^a_{t} \vert o^a_{t}} $, but this is not the case in our problem (the state and action spaces may not even be the same). 
Just to illustrate, if we have a fully observed game, then we know that $\prob{o^e_t \vert o^a_t, a^a_t}$ is the indicator for the environment state's observation, which the agent can deduce. 
Then Equation \ref{eq:markov-breakdown} simplifies to just understanding the environment's policy. 
\begin{equation}
	\prob{o^a_{t+1} \vert o^a_t, a^a_t} = \sum_{a^e_t} \prob{a^e_{t} \vert o^e_{t}} \prob{o^a_{t+1} \vert o^e_t, a^e_t}
	\label{eq:observed}
\end{equation}

So, we define a hidden human state $\{h_t : t \in \{1, \dots, T\}\}$. We want to see if the inclusion of this human hidden state
can help us better understand the environment. In the event of infinite multiversal simulation data on the entire population, we can view $h$ as the selector 
of the specific person in a population. However, in our case, we only have a small amount of data per person, so we can only view $h$ as a
selector of a sub-population. In the worst case, $T = 1$ could imply that there is no further information we can gather from the person about how 
they play the game and we can only rely on the population information that we have. 
Using this, we can potentially estimate the environment's policy as
\begin{equation}
	q(o^a_t, a^a_t, h_t) \approx \prob{ o^e_t \vert o^a_t, a^a_t} \prob{a^e_{t} \vert o^e_{t}}
	\label{eq:problem}
\end{equation}

The inclusion of $h$ does complicate things, though, as it introduces a second level of dynamics and, thus, a second level of estimation uncertainty. 
If we were to do the estimation, $h_t$ can depend on the entire history of the game, \textit{i.e.} $\prob{h_{t+1} \vert h_{1:t}, o^e_{1:t}, r^e_{1:t}}$, and 
perhaps even to previous plays of this game or other games. Even if only a fixed window affects the history, this adds to the difficulty to estimate. 
Furthermore, even if we were to have all the game data, we would still have to either use unsupervised learning techniques to assign values of $h$ or use some other form of prior knowledge.
Thus, we have to choose the possible modeling of $h_t$ conservatively based on the data that we have in order to provide the best possible estimate provided in Equation \ref{eq:problem}. 
As a step toward this direction, we allow the ability to try and get access to $h_t$ through interventions, such as by asking a student about how they are studying. 

Now we can add the rewards back in to picture. In our case, currently the reward will depend only on the action taken $a^a_t$ and the next observation $o^a_{t+1}$, but to be more general we can also define
\begin{equation}
 	r(o^a_t, a^a_t, h_t) \approx \prob{r^a_{t+1} \vert o^a_t, a^a_t}
 	\label{eq:reward}
\end{equation}
and therefore, our final objective will be the same as most RL problems with maximizing the aggregate expected reward
\begin{equation}
	G^a_t = \sum_{k=t+1}^T \gamma^{k-(t+1)} r^a_{k}
\end{equation}
at any point in time, where $\gamma$ is the RL discount factor to balance short and long-term rewards. 

One other differentiating factor we want to consider in our problem is the inclusion of interventions. 
On one hand, one can view the ``exploration" steps in RL to be probing interventions, as we are choosing to step away from the currently found optimal policy to see if there are other solutions. 
On the other, we can also direclty impose extra interventions, 
actions that are not part of the ``basic" set of actions in the game space that would change the state in a way that would normally follow the game rules (usually with a cost in reward to make the game actions separate). 
From the perspective of information flow, typically inclusion of probing interventions is an interesting way of changing the environment toward providing better collaboration, even if the probing intervention has a cost. 

Another way this can be seen is that its changing into a similar, but different version of the game. 
The idea is that most of the concepts should still transfer between these versions of the game, but may now have extra tools to attempt to earn the highest reward. 

\begin{figure}[htbp]
	\begin{center}
		\input tikz/problem.tikz
	\end{center}
	\caption{A simple hypothesized DAG about how a student may produce results for any single concept in a duration of time. Each of the inputs at the top are time dependent. }
	\label{fig:problem}
\end{figure}

